SemGloVe: Semantic Co-occurrences for GloVe from BERT

GloVe learns word embeddings by leveraging statistical information from word co-occurrence matrices. However, word pairs in the matrices are extracted from a predefined local context window, which might lead to limited word pairs and potentially semantic irrelevant word pairs. In this paper, we propose SemGloVe, which distills semantic co-occurrences from BERT into static GloVe word embeddings. Particularly, we propose two models to extract co-occurrence statistics based on either the masked language model or the multi-head attention weights of BERT. Our methods can extract word pairs without limiting by the local window assumption and can define the co-occurrence weights by directly considering the semantic distance between word pairs. Experiments on several word similarity datasets and four external tasks show that SemGloVe can outperform GloVe.

==> figures/DevDim.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/GraphDim.eps}
	\caption{Development evaluation On WS353S against vector  dimension.}
	\label{dev::dimension}
\end{figure}

\iffalse
\begin{figure*}[t]
    \centering
    \subfigure[Masked Language Model]{
        \begin{minipage}{7cm}
        \centering
        \includegraphics[width=1.0\textwidth]{figures/mlm.png}
        \end{minipage}
    }
    \subfigure[Self Attention Network]{
        \begin{minipage}{7cm}
        \centering
        \includegraphics[width=1.0\textwidth]{figures/self_attention_scores.png}
        \end{minipage}
    }
	\label{Model Architecture}
	\caption{Two methods to distill semantic co-occurrences from BERT.}
\end{figure*}
\fi

==> figures/corpusSize.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/GraphCorpus.eps}
	\caption{Development evaluation On WS353S against corpus size.}
	\label{dev::corpus}
\end{figure}

==> figures/wordPairCount.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/wordPairCount.eps}
	\caption{Average word-word co-occurrence counts of GloVe and SemGloVe.}
	\label{figure:analysis:averagewordCount}
\end{figure}

==> tables/countcontrol.tex <==
\begin{table}[t]
\footnotesize
\centering
\begin{tabular}{|l|c|c|c|c|}
\hline

\textbf{Models} & \textbf{WS353} & \textbf{WS353S} & \textbf{WS353R} & \textbf{SimLex999} \\ \hline
GloVe     &52.6 & 62.3     & 55.5   & 28.2 \\
san\_div & 56.0 & 65.9 & 56.3 & 31.9 \\
mlm\_div & 66.6 & 74.9 & 61.9 & \textbf{44.7} \\ \hline
san\_div\_fill & 52.7 & 60.5 & 54.6 & 27.7 \\
mlm\_div\_fill & - & - & - & - \\
\hline
\end{tabular}
\caption{SemGloVe Intrinsic Evaluation: Comparision on WS353, WS353S, WS353R and SimLex999 datasets.} 
\label{tab:analysis:control}
\end{table}

==> tables/devontonote.tex <==
\begin{table}[!t]
    \centering
    \footnotesize
	\begin{tabular}{|l|c|c|c|c|}
		\hline \textbf{Models}&\textbf{P}& \textbf{R}& \textbf{Dev-F1}&\textbf{Test-F1}\\
		\hline
		add\_one\_tune&74.18&71.11&72.61&74.49\\
		softmax\_tune&74.94&71.02&72.92&\textbf{74.98}\\
		ratio\_tune&73.80&72.03&72.90&74.30\\
		reciprocal\_tune&75.03&71.91&\textbf{73.44}&74.68\\
		add\_one\_fix&73.70&72.83&73.27&74.46\\
		softmax\_fix&73.20&72.44&72.82&74.19\\
		ratio\_fix&73.42&73.77&73.59&75.00\\
		reciprocal\_fix&73.65&73.88&\textbf{73.77}&\textbf{75.35}\\
		\hline
	\end{tabular}
	\caption{Dev results on Chiense OntoNotes.} \label{tab:dev:ontonote}
\end{table}

==> tables/devxmax.tex <==
\begin{table}[t]
\scriptsize
\centering
\begin{tabular}{|l|c|c|c|c|c|}
\hline
\textbf{Models}& $x_{\text{max}}$=1 & $x_{\text{max}}$=10 & $x_{\text{max}}$=20 & $x_{\text{max}}$=50 & $x_{\text{max}}$=100 \\ \hline
GloVe     & 59.93 & 62.30 & 61.36 & 61.22 & 61.14 \\ \hline
SemGloVe_\text{sr} & 60.30 & 62.80 & 62.00 & 61.37 & 60.61 \\
SemGloVe_\text{sd} & 60.96 & 65.90 & 61.62 & 61.82 & 60.34 \\
SemGloVe_\text{mr} &73.60 &78.00 &74.69 &76.30 &77.63  \\
SemGloVe_\text{md} &75.93 &74.90 &74.01 &73.27 &75.89\\
\hline
\end{tabular}
\caption{Results on WS353S with different $x_\text{max}$ value.} 
\label{tab:dev:xmax}
\end{table}

==> tables/docqa.tex <==
\begin{table}[!t]
    \centering
    \footnotesize
	\begin{tabular}{|l|c|c|c|c|}
		\hline \textbf{Models}&\textbf{Train-F1}&\textbf{Dev-F1}\\
		\hline
		base\_glove\_tune& 78.61 & 78.71 \\
		word\_bpe\_tune& 79.63 & 80.00 \\
		geomean\_tune& \textbf{79.86} & \textbf{80.03} \\
		arithmean\_tune& 79.48 & 79.74 \\
		\hline
	\end{tabular}
	\caption{Main results on the standard SQuAD datasets.} 
	\label{tab:dev:en:pos}
\end{table}

==> tables/downstream.tex <==
\iffalse
\begin{table}[t]
\scriptsize
\centering
\begin{tabular}{|l|c|c|c|c|c|}
\hline
\textbf{Models} & \textbf{CCG} & \textbf{QA} & \textbf{Co-Ref} & \textbf{NER} & \textbf{Average} \\ \hline
Word2Vec           & 94.29 & 79.66 & 72.07  & 86.66 & 83.17 \\
Fasttext           & 94.24  & 80.34 & 72.35 & 86.74 & 83.42 \\ 
SynGCN             & 94.35  & 80.24 & 72.11 & 87.50 & 83.55 \\
SemGCN             & 94.66  & 79.94 & 71.88 & 86.81 & 83.32 \\
\hline

GloVe     &94.40  & 79.04 & 71.93 & 86.72 & 82.77 \\ 
GloVe$_\text{6B}$     & 94.39 & 79.72 & 71.58 & 87.15 & 83.21 \\ \hline

SemGloVe_{sr} & \textbf{94.52}  & 79.12 &  72.08 & 86.99 & 83.18\\
SemGloVe_{sd} & 94.51 & 79.02 & 72.21 & \textbf{87.05} & 83.20 \\

SemGloVe_{mr} & 94.43 & \textbf{80.37} & \textbf{72.25} & 86.38 & \textbf{83.36} \\

SemGloVe_{md} & 94.35 & 80.16 & 72.14 & 86.33 & 83.25 \\
\hline
BERT_{large} & - & 90.90 & 77.10 & 89.16 & - \\
\hline
\end{tabular}
\caption{Extrinstic Evaluation: Comparison on CCG, QA, Co-Ref and NER tasks. The bold results are the best results of SemGloVe.} 
\label{tab:main:downstream}
\end{table}

\fi
\iffalse
\begin{table}[t]
\scriptsize
\centering
\begin{tabular}{|l|c|c|c|c|}
\hline
\textbf{Models} & \textbf{CCG} & \textbf{QA} & \textbf{Co-Ref} & \textbf{Average} \\ \hline
Word2Vec           & 94.29 & 79.66 & 72.07  & 83.17 \\
Fasttext           & 94.24  & 80.34 & 72.35 & 83.42 \\ 
SynGCN             & 94.35  & 80.24 & 72.11 & 83.55 \\
SemGCN             & 94.66  & 79.94 & 71.88 & 83.32 \\
\hline

GloVe     &94.40  & 79.04 & 71.93 & 82.77 \\ \hline

SemGloVe_{sr} & \textbf{94.52}  & 79.12 & 72.08 & 83.18\\
SemGloVe_{sd} & 94.51 & 79.02 & 72.21 & 83.20 \\

SemGloVe_{mr} & 94.43 & \textbf{80.37} & \textbf{72.25} & \textbf{83.36} \\

SemGloVe_{md} & 94.35 & 80.16 & 72.14 & 83.25 \\

\hline
\end{tabular}
\caption{Extrinstic Evaluation: Comparison on CCG, QA and Co-Ref tasks. The bold results are the best results of SemGloVe.} 
\label{tab:main:downstream}
\end{table}
\fi
\iffalse
average with ner
82.01
82.31
82.23
82.16
81.79
81.91
81.91
82.35
82.22
\fi

==> tables/mainccg.tex <==
\begin{table}[!t]
    \centering
    \footnotesize
	\begin{tabular}{|l|c|c|c|c|}
		\hline \textbf{Models}&\textbf{Dev-Accuracy}&\textbf{Test-Accuracy}\\
		\hline
		base\_glove\_tune&94.28&94.24\\
		geomean\_fix& 94.08 & 94.16 \\
		arithmean\_fix& 93.89 &94.12\\
		word\_bpe\_tune& \textbf{94.57} & 94.42 \\
		geomean\_tune& 94.25 & 94.34 \\
		arithmean\_tune&94.23&\textbf{94.46}\\
		\hline
	\end{tabular}
	\caption{Main results on CCG.} 
	\label{tab:dev:en:ontonote}
\end{table}

==> tables/maincoref.tex <==
\begin{table}[!t]
    \centering
    \footnotesize
	\begin{tabular}{|l|c|c|}
		\hline \textbf{Models}&\textbf{Dev-F1}&\textbf{Test-F1}\\
		\hline
		base\_glove\_tune & 72.24 & 71.78 \\
		san\_recip\_tune & - & - \\
		san\_divide\_tune & - & - \\
		mlm\_recip\_tune& - & - \\
		mlm\_divide\_tune& - & - \\
		\hline
	\end{tabular}
	\caption{Main results on CONLL-2012 Coreference Resolution Task.} 
	\label{tab:dev:coref}
\end{table}

==> tables/mainenontonote.tex <==
\begin{table}[!t]
    \centering
    \footnotesize
	\begin{tabular}{|l|c|c|c|c|}
		\hline \textbf{Models}&\textbf{P}& \textbf{R}& \textbf{Dev-F1}&\textbf{Test-F1}\\
		\hline
		base\_glove\_tune&84.64&86.66&85.64&87.17\\
		geomean\_tune&84.57&85.95&85.25&86.68\\
		arithmean\_tune&84.08&86.39&85.22&86.66\\
		geomean\_fix&83.51&85.52&84.50&85.90\\
		arithmean\_fix&82.84&85.90&84.34&85.94\\
		\hline
	\end{tabular}
	\caption{Main results on English OntoNotes.} \label{tab:dev:en:ontonote}
\end{table}

==> tables/mainmsra.tex <==
\begin{table}[!t]
	\centering
	\footnotesize
	\begin{tabular}{|l|c|c|c|}
		\hline \textbf{Models}&\textbf{P}& \textbf{R}& \textbf{F1}\\
		\hline
		word2vec\_tune& 93.28 & 92.77 & 93.02 \\
		base\_glove\_tune&93.14&92.97&93.05\\
		bert\_glove\_tune&93.03&93.11&93.07\\
		word2vec\_fix& 92.95 & 92.17 & 92.56 \\
		base\_glove\_fix&92.96&92.31&92.63\\		bert\_glove\_fix&93.15&93.17&\textbf{93.16}\\
		\hline
	\end{tabular}
	\caption{Main results on MSRA}
	\label{tab:main:msra}
\end{table}

==> tables/mainontonote.tex <==
\begin{table}[!t]
	\centering
	\footnotesize
	\begin{tabular}{|l|c|c|c|}
		\hline \textbf{Models}&\textbf{P}& \textbf{R}& \textbf{F1}\\
		\hline
		word2vec\_tune&73.49&75.19&74.33\\
		base\_glove\_tune&74.01&72.13&73.06\\
		bert\_glove\_tune&75.01&73.60&74.30\\
		word2vec\_fix&73.37&75.01&74.18\\
		base\_glove\_fix&72.00&73.97&72.97\\		bert\_glove\_fix&74.52&75.48&\textbf{75.00}\\
		\hline
	\end{tabular}
	\caption{Main results on Chinese OntoNotes}
	\label{tab:main:ontonote}
\end{table}

==> tables/mainpos.tex <==
\begin{table}[!t]
    \centering
    \footnotesize
	\begin{tabular}{|l|c|c|c|c|}
		\hline \textbf{Models}&\textbf{Dev-Accuracy}&\textbf{Test-Accuracy}\\
		\hline
		base\_glove\_tune& 97.59 & 97.52 \\
		geomean\_fix& 97.55 & 97.47 \\
		arithmean\_fix& 97.57 & 97.48 \\
		geomean\_tune& 97.55 & 97.53 \\
		arithmean\_tune& 97.54 & 97.48 \\
		\hline
	\end{tabular}
	\caption{Dev results on POS.} 
	\label{tab:dev:en:pos}
\end{table}

==> tables/mainresume.tex <==
\begin{table}[!t]
	\centering
	\footnotesize
	\begin{tabular}{|l|c|c|c|}
		\hline \textbf{Models}&\textbf{P}& \textbf{R}& \textbf{F1}\\
		\hline
		word2vec\_tune& 93.53 & 94.05 & 93.79 \\
		base\_glove\_tune&94.48&94.42&94.45\\
		bert\_glove\_tune&94.14&94.60&94.37\\
		word2vec\_fix& 94.76 & 94.29 & 94.53 \\
		base\_glove\_fix&94.90&94.85&94.88\\
		bert\_glove\_fix&95.27&95.15&\textbf{95.21}\\
		\hline
	\end{tabular}
	\caption{Main results on Resume}
	\label{tab:main:resume}
\end{table}

==> tables/mainsnli.tex <==
\begin{table}[!t]
    \centering
    \footnotesize
	\begin{tabular}{|l|c|c|c|c|}
		\hline \textbf{Models}&\textbf{Dev-Accuracy}&\textbf{Test-Accuracy}\\
		\hline
		base\_glove\_tune& 86.79 & 86.11 \\
		word\_bpe\_tune& \textbf{87.10} & 85.91 \\
		arithmean\_tune& 86.76 & 86.03 \\
		geomean\_tune& 86.99 & \textbf{86.59} \\
		\hline
	\end{tabular}
	\caption{Main results on SNLI.} 
	\label{tab:dev:snli}
\end{table}

==> tables/mainweibo.tex <==
\begin{table}[!t]
	\centering
	\footnotesize
	\begin{tabular}{|l|c|c|c|}
		\hline \textbf{Models}&\textbf{NE}& \textbf{NM}& \textbf{Overall}\\
		\hline
		word2vec& - & - & - \\
		base\_glove\_tune& - & - &\textbf{53.28}\\
		bert\_glove\_tune& - & - &52.60\\
		base\_glove\_fix& - & - &48.18\\
		bert\_glove\_fix& - & - &\textbf{50.29}\\
		\hline
	\end{tabular}
	\caption{Main results on Weibo NER}
	\label{tab:main:weibo}
\end{table}

==> tables/similarity.tex <==
\begin{table}[t]
\scriptsize
\centering
\begin{tabular}{|l|c|c|c|c|c|}
\hline
\textbf{Models} & \textbf{W353} & \textbf{W353S} & \textbf{W353R} & \textbf{SL999} & \textbf{Average}\\ \hline
Word2Vec                 & 61.6 & 69.2 & 54.6 & 35.1 & 52.6 \\
Deps               & 60.6 & 65.7 & 36.2 & 39.6 & 50.5 \\
Fasttext           &68.3      & 74.4    & 65.4   & 34.9 & 60.8 \\ 
SynGCN             &60.9      & 73.2    & 45.7   & 45.5 & 56.3 \\
SemGCN  &  60.9 &  65.9  &  60.3  & 48.8 & 59.0 \\\hline

GloVe     &52.6 & 62.3 & 55.5   & 28.2 & 49.7 \\ 
GloVe_\text{6B} & 56.5 & 64.6 & 50.0 & 31.3 & 50.6 \\\hline

SemGloVe_{sr} & 54.0 & 62.8 & 54.9 & 29.3 & 50.3 \\
SemGloVe_{sd} & 56.0 & 65.9 & 56.3 & 31.9 & 52.5 \\

SemGloVe_{mr} & 65.2 & \textbf{78.0} & 59.7 & 43.9 & 61.7 \\
SemGloVe_{md} & \textbf{66.6} & 74.9 & \textbf{61.9} & \textbf{44.7} & \textbf{62.0} \\

\hline
\end{tabular}
\caption{Intrinsic Evaluation: Comparison on WS353 (W353) and SimLex999 (SL999) datasets. The bold results are the best results of SemGloVe.} 
\label{tab:main:results}
\end{table}

==> tables/totalpaircount.tex <==
\begin{table*}[!t]
	\centering
	\begin{tabular}{|l|c|c|c|c|c|}
		\hline \textbf{Methods}&GloVe&SemGloVe_{sr}&SemGloVe_{sd}&SemGloVe_{mr}&SemGloVe_{md}\\
		\hline
		Count $>$ 0 & 13.39 & 13.81 & 19.41 & 5663.45 & 5335.49 &
		Count $>$ 1 & 42.86 & 53.30 & 57.16 & 9152.59 & 7531.51 & 
		Count $>$ 10 & 214.09  & 262.15 & 279.78 & 16560.29 & 13581.92 & 
		Count $>$ 100 & 1231.71 & 1428.34 & 1520.04 & 34744.91 & 28412.04 & 
		Count $>$ 1000 & 7546.35 & 8187.79 & 8731.19 & 86060.60 & 70187.52 & 
		Count $>$ 10000 & 47329.65 & 53203.14 & 55124.44 & 254565.69 & 210829.83 &  
		\hline
	\end{tabular}
	\caption{Total word-word co-occurrence counts of GloVe and SemGloves.}
	\label{tab:analysi:totalcount}
\end{table*}

\iffalse
\hline
		Count $>$ 0 & 345M & 204M(13.81) & 204M(19.41) & 150M & 150M &
		Count $>$ 1 & 105M (105412725) & 51M(51833056)(53.30) & 68241364(57.16) & (90268285) & 107M & 
		Count $>$ 10 & 20M(19909695)  & 10M (10065953)(262.15) & (13361404)(279.78) & (49880832) & 59M & 
		Count $>$ 100 & 3M(3072461) & 1.7M(1679206)(1428.34) & (2249104)(1520.04) & (23747804) & 28M & 
		Count $>$ 1K & 0.41M(405836) & 0.24M(244172)(8187.79) & (330576)(8731.19) & (9530772) & 11M & 
		Count $>$ 10K & 0.044M(44326)(47329.65) & 0.026M(26498)(53203.14) & (37902)(55124.44) & (3138421) & 3.6M &  
		\hline
1	42.86	53.3	57.16	9152.59	7531.51
1000	7546.35	8187.79	8731.19	86060.6	70187.52
10000	47329.65	53203.14	55124.44	254565.69	210829.83
\fi

==> tables/wordanalogies.tex <==
\begin{table*}[h]
\scriptsize
\centering
\begin{tabular}{lcccc|cccc|cc}
\hline
                   & \multicolumn{4}{c|}{Word Similarity} & \multicolumn{4}{c|}{Concept Categorization} & \multicolumn{2}{c}{Word Analogy} \\ \cline{2-11} 
Method             & WS353S  & WS353R & SimLex999 & RW   & AP      & Battings    & BLESS    & ESSLI    & SemEval2012         & MSR         \\ \hline
Word2Vec           & 71.4    & 52.6   & 38.0      & 20.0 & 63.2    & 43.3        & 77.8     & 63.0     & 18.9                & 44.0        \\
GloVe              & 69.2    & 53.4   & 36.7      & 29.6 & 58.0    & 41.3        & 80.0     & 59.3     & 18.7                & 45.8        \\
Deps               & 65.7    & 36.2   & 39.6      & 33.0 & 61.8    & 41.7        & 65.9     & 55.6     & 22.9                & 40.3        \\
EXT                & 69.6    & 44.9   & 43.2      & 18.6 & 52.6    & 35.0        & 65.2     & 66.7     & 21.8                & 18.8        \\
SynGCN             & 73.2    & 45.7   & 45.5      & 33.7 & 69.3    & 45.2        & 85.2     & 70.4     & 23.4                & 52.8        \\
Fasttext           & 74.4    & 65.4   & 34.9      & 40.1 & 65.0    & 44.6        & 78.0     & 73.1     & 17.7                & 53.3        \\ \hline
word2vec\_word      &71.2     & 64.8   & 35.9      & 37.8 & 63.6    & 43.8        & 74.4     & 74.4     & 13.5                & 48.0   \\
baseglove\_word       &61.8     & 54.5   & 27.4      & 32.5 & 48.6    & 31.7        & 68.3     & 71.8     & 12.9                & 40.8   \\
baseglove\_bpe       &55.6     & 57.1   & 31.3      & 28.1 & 43.6    & 28.7        & 58.5     & 66.9     & 17.8                & 36.5   \\
mlm\_reciprocal\_bpe       &80.2     & 61.7   & 50.0      & 29.7 & 45.0    & 24.7        & 63.4     & 70.5     & 16.6                & 45.3   \\
mlm\_reciprocal\_average\_bpe       &82.6     & 58.6   & 49.2      & 23.1 & 47.1    & 25.1        & 63.4     & 70.5     & 11.7                & 18.1   \\
mlm\_reciprocal & 76.5 & 58.75 & 44.93 & 19.67 & 44.3 & 25.0 & 58.5 & 67.9 & 12.1 & 35.9 \\
mlm\_reciprocal\_arithmean & 75.5 & 58.4 & 40.7 & 25.4 & 45.0 & 26.1 & 58.5 & 73.0 & 13.1 & 38.4 \\
mlm\_reciprocal\_geomean & 73.8 & 66.1 & 40.4 & 29.6 & 43.6 & 25.2 & 59.8 & 69.7 & 7.9 & 40.1 \\

mlm\_divide & 77.5 & 60.11 & 44.77 & 21.15 & 44.3 & 27.4 & 69.5 & 66.8 & 5.6 & 44.6 \\

\hline
\end{tabular}
\end{table*}

%
%glove\_word\_count\_bpe: constructing word pair count from bpes pair count \\
%base\_glove\_word\_count\_nobpe: removing word pairs which having no bpe pairs beween them \\
%base\_glove\_word\_bpeword\_arithmean: merge base glove word pair with constructing word pairs \\ %using arith mean


% \begin{table}[h]
% 	\centering
% 	\begin{tabular}{|l|c|c|c|}
% 		\hline \textbf{Models}&\textbf{Dim}&\textbf{Add}& \textbf{Mul}\\
% 		\hline
% 		word2vec&50&0.05&0.03\\
% 		base\_glove&50&0.12&0.07\\
% 		bert\_glove&50&\textbf{0.19}&\textbf{0.11}\\
% 		\hline
% 	\end{tabular}
% 	\caption{Main results on Word Analogies}
% 	\label{tab:main:wordanalogies}
% \end{table}
